Probing the circumgalactic medium with CMB polarization statistical anisotropy

As cosmic microwave background (CMB) photons traverse the Universe, anisotropies can be induced via Thomson scattering (proportional to the integrated electron density; optical depth) and inverse Compton scattering (proportional to the integrated electron pressure; thermal Sunyaev-Zel'dovich effect). Measurements of anisotropy in optical depth $\tau$ and Compton $y$ parameter are imprinted by the galaxies and galaxy clusters and are thus sensitive to the thermodynamic properties of circumgalactic medium and intergalactic medium. We use an analytic halo model to predict the power spectrum of the optical depth ($\tau\tau$), the cross-correlation between the optical depth and the Compton $y$ parameter ($\tau y$), as well as the cross-correlation between the optical depth and galaxy clustering ($\tau g$), and compare this model to cosmological simulations. We constrain the optical depths of halos at $z\lesssim 3$ using a technique originally devised to constrain patchy reionization at a much higher redshift range. The forecasted signal-to-noise ratio is 2.6, 8.5, and 13, respectively, for a CMB-S4-like experiment and a VRO-like optical survey. We show that a joint analysis of these probes can constrain the amplitude of the density profiles of halos to 6.5% and the pressure profile to 13%, marginalizing over the outer slope of the pressure profile. These constraints translate to astrophysical parameters related to the physics of galaxy evolution, such as the gas mass fraction, $f_{\rm g}$, which can be constrained to 5.3% uncertainty at $z\sim 0$, assuming an underlying model for the shape of the density profile. The cross-correlations presented here are complementary to other CMB and galaxy cross-correlations since they do not require spectroscopic galaxy redshifts and are another example of how such correlations are a powerful probe of the astrophysics of galaxy evolution.

==> CGM/macros.tex <==
\def\Planck{\textit{Planck}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bga}{\begin{gathered}}
\newcommand{\ega}{\end{gathered}}

\newcommand{\fnl}{f_{\rm{NL}}}
\newcommand{\fnlloc}{f^{\rm local}_{\rm NL}}
\newcommand{\fnleqi}{f^{\rm equil}_{\rm NL}}
\newcommand{\taunl}{\tau_{\rm{NL}}}
\newcommand{\gnl}{g_{\rm{NL}}}
\newcommand{\htaunl}{\hat{\tau}_{\rm NL}}
\newcommand{\barmodulation}{\bar{f}}
\newcommand{\hatmodulation}{\hat{f}}
\newcommand{\mfmodulation}{\barmodulation^{\rm MF}}
\newcommand{\hatReconNoise}{\hat{N}_L}
\providecommand{\fsky}{f_{\rm sky}}
\newcommand{\fskyeff}{\fsky^{\rm eff}}

\providecommand{\planck}{\textit{Planck}}

\newcommand{\covinvT}{\bar{T}}
\newcommand{\Ltemp}{\tilde{T}}
\newcommand{\lensedC}{\tilde{C}}
\newcommand{\Lmin}{{L_{\rm min}}}
\newcommand{\Lmax}{{L_{\rm max}}}

\providecommand{\alt}{\lea}
\providecommand{\agt}{\gea}

\providecommand{\LCDM}{{$\rm{\Lambda CDM}$}}


\newcommand\ba{\begin{eqnarray}}
\newcommand\ea{\end{eqnarray}}
\newcommand\bea{\begin{eqnarray}}
\newcommand\eea{\end{eqnarray}}

\newcommand\be{\begin{equation}}
\newcommand\ee{\end{equation}}


%Variance
\providecommand{\var}{\text{var}}
%covariance
\providecommand{\cov}{\text{cov}}

%integration
\newcommand{\ud}{{\rm d}}

%Other
\newcommand{\tauy}{\langle \tau \rangle-\langle y \rangle}
\newcommand{\tauM}{\langle \tau \rangle-M}
\newcommand{\rmn}{\mathrm}

%%%%%%%% Vectors %%%%%%%%%%

%\newcommand{\boldvec}[1]{{{\mathbf{#1}}}}

\newcommand{\boldvec}[1]{{{\vec{#1}}}}

\newcommand{\vA}{\boldvec{A}}
\newcommand{\vB}{\boldvec{B}}
\newcommand{\vC}{\boldvec{C}}
\newcommand{\vD}{\boldvec{D}}
\newcommand{\vE}{\boldvec{E}}
\newcommand{\vF}{\boldvec{F}}
\newcommand{\vG}{\boldvec{G}}
\newcommand{\vH}{\boldvec{H}}
\newcommand{\vI}{\boldvec{I}}
\newcommand{\vJ}{\boldvec{J}}
\newcommand{\vK}{\boldvec{K}}
\newcommand{\vL}{\boldvec{L}}
\newcommand{\vM}{\boldvec{M}}
\newcommand{\vN}{\boldvec{N}}
\newcommand{\vO}{\boldvec{O}}
\newcommand{\vP}{\boldvec{P}}
\newcommand{\vQ}{\boldvec{Q}}
\newcommand{\vR}{\boldvec{R}}
\newcommand{\vS}{\boldvec{S}}
\newcommand{\vT}{\boldvec{T}}
\newcommand{\vU}{\boldvec{U}}
\newcommand{\vV}{\boldvec{V}}
\newcommand{\vW}{\boldvec{W}}
\newcommand{\vX}{\boldvec{X}}
\newcommand{\vY}{\boldvec{Y}}
\newcommand{\vZ}{\boldvec{Z}}

\newcommand{\va}{\boldvec{a}}
\newcommand{\vb}{\boldvec{b}}
\newcommand{\vc}{\boldvec{c}}
\newcommand{\vd}{\boldvec{d}}
\newcommand{\ve}{\boldvec{e}}
\newcommand{\vf}{\boldvec{f}}
\newcommand{\vg}{\boldvec{g}}
\newcommand{\vh}{\boldvec{h}}
\newcommand{\vi}{\boldvec{i}}
\newcommand{\vj}{\boldvec{j}}
\newcommand{\vk}{\boldvec{k}}
\newcommand{\vl}{\boldvec{l}}
\newcommand{\vm}{\boldvec{m}}
\newcommand{\vn}{\boldvec{n}}
\newcommand{\vo}{\boldvec{o}}
\newcommand{\vp}{\boldvec{p}}
\newcommand{\vq}{\boldvec{q}}
\newcommand{\vs}{\boldvec{s}}
\newcommand{\vt}{\boldvec{t}}
\newcommand{\vu}{\boldvec{u}}
\newcommand{\vv}{\boldvec{v}}
\newcommand{\vw}{\boldvec{w}}
\newcommand{\vx}{\boldvec{x}}
\newcommand{\vy}{\boldvec{y}}
\newcommand{\vz}{\boldvec{z}}

\newcommand{\cla}{\mathcal{A}}
\newcommand{\clb}{\mathcal{B}}
\newcommand{\clc}{\mathcal{C}}
\newcommand{\cld}{\mathcal{D}}
\newcommand{\cle}{\mathcal{E}}
\newcommand{\clf}{\mathcal{F}}
\newcommand{\clg}{\mathcal{G}}
\newcommand{\clh}{\mathcal{H}}
\newcommand{\cli}{\mathcal{I}}
\newcommand{\clj}{\mathcal{J}}
\newcommand{\clk}{\mathcal{K}}
\newcommand{\cll}{\mathcal{L}}
\newcommand{\clm}{\mathcal{M}}
\newcommand{\cln}{\mathcal{N}}
\newcommand{\clo}{\mathcal{O}}
\newcommand{\clp}{\mathcal{P}}
\newcommand{\clq}{\mathcal{Q}}
\newcommand{\clr}{\mathcal{R}}
\newcommand{\cls}{\mathcal{S}}
\newcommand{\clt}{\mathcal{T}}
\newcommand{\clu}{\mathcal{U}}
\newcommand{\clv}{\mathcal{V}}
\newcommand{\clw}{\mathcal{W}}
\newcommand{\clx}{\mathcal{X}}
\newcommand{\cly}{\mathcal{Y}}
\newcommand{\clz}{\mathcal{Z}}



\newcommand{\vnhat}{\hat{\vn}}
\newcommand{\vrhat}{\hat{\vr}}
\newcommand{\vkhat}{\hat{\vk}} 


%%% compon separat%%%%%
\def\Commander{\texttt{Commander}}
\def\Ruler{\texttt{Ruler}}
\def\CR{\texttt{C-R}}
\def\NILC{\texttt{NILC}}
\def\SMICA{\texttt{SMICA}}
\def\SEVEM{\texttt{SEVEM}}

%%%%%% Math symbols %%%%%%
\def\hf{\frac{1}{2}}
\def\pl{\parallel}
\def\pp{\bot}
\def\px{\approx}
\def\pr{\prime}

%%%%%% Align symbols %%%%%%
\def\={\nonumber &=}
\def\nn{\nonumber}
%\def\&{{}&}

%%%%%% Brackets %%%%%%
\def\({\left(}
\def\){\right)}
\def\[{\left[}
\def\]{\right]}
\def\<{\left\langle}
\def\>{\right\rangle}



%%%%%% Vectors %%%%%%
\def\uk{{\bf \hat{k}}}
\def\un{{\bf \hat{n}}}
\def\ur{{\bf \hat{r}}}
\def\ux{{\bf \hat{x}}}
\def\bk{{\bf k}}
\def\bn{{\bf n}}
\def\br{{\bf r}}
\def\bv{{\bf v}}
\def\bx{{\bf x}}
\def\bl{{\bf l}}
\def\bkp{{\bf k^\pr}}
\def\brp{{\bf r^\pr}}


%%%%%% Shortcuts for commands %%%%%%
\def\bib{\bibitem}
\def\curl{\mathcal}
\def\nl{\nonumber &=&}
\def\eq{\begin{eqnarray}}
\def\qe{\end{eqnarray}}

\def\and{\quad \mbox{and} \quad}
\def\imp{\quad \Rightarrow \quad}

%%%%%% shortcuts for environments %%%%%%
\newenvironment{mylist}{\begin{list}
    {$\bullet$}
    {\setlength{\leftmargin}{1cm}
    \setlength{\rightmargin}{1cm}
    \setlength{\labelsep}{.5cm}
    \setlength{\itemsep}{.5cm}}}
{\end{list}}

%%%%%% other abbreviations %%%%%%
\def\spie{Proc.\ SPIE}

%%%%%% Bispectrum abbreviations %%%%%%
\def\fnl{f_\textrm{NL}}
\def\barfnl{\bar f_\textrm{NL}}
\def\Fnl{ F_\textrm {NL}}
\def\barFnl{ \bar F_\textrm {NL}}
\def\Fnllocal{F_\textrm {NL}^\textrm{local}}
\def\fnllocal{f_\textrm {NL}^\textrm{local}}
\def\Fnlequil{F_\textrm {NL}^\textrm{equil}}
\def\fnlequil{f_\textrm {NL}^\textrm{equil}}
\def\Fnlequil{F_\textrm {NL}^\textrm{dbi}}
\def\fnlequil{f_\textrm {NL}^\textrm{dbi}}
\def\Fnlfeat{F_\textrm {NL}^\textrm{feat}}
\def\fnlfeat{f_\textrm {NL}^\textrm{feat}}
\def\Fnlmodel{F_\textrm {NL}^\textrm{model}}
\def\fnlmodel{f_\textrm {NL}^\textrm{model}}
\def\Fnlth{F_\textrm {NL}^\textrm{th}}
\def\fnlth{f_\textrm {NL}^\textrm{th}}
\def\bfnl{\kern2pt\overline{\kern-2ptf}_\textrm{NL}}

\def\lmax{\ell_\textrm{max}}
\def\lall{\ell_1,\ell_2,\ell_3}
\def\lalltwo{\ell_4,\ell_5,\ell_6}
\def\lsum{\ell_1+\ell_2+\ell_3}
\def\ltilde{\tilde l}
\def\Blll{B_{\ell_1\ell_2\ell_3}}
\def\blll{b_{\ell_1\ell_2\ell_3}}
\def\bllllocal{b_{\ell_1\ell_2\ell_3}^\textrm{local}}
\def\blllmodel{b_{\ell_1\ell_2\ell_3}^\textrm{model}}
\def\blllconst{b_{\ell_1\ell_2\ell_3}^\textrm{const}}
\def\blllequil{b_{\ell_1\ell_2\ell_3}^\textrm{equil}}
\def\blllstring{b_{\ell_1\ell_2\ell_3}^\textrm{string}}
\def\hlll{h_{\ell_1\ell_2\ell_3}}
\def\hllltwo{h_{\ell_4\ell_5\ell_6}}

\def\th{\textrm{th}}
\def\exp{\textrm{exp}}

\def\kmax{k_\textrm{max}}
\def\kall{k_1,k_2,k_3}
\def\ksum{k_1+k_2+k_3}
\def\ktilde{\tilde k}
\def\bfkall{\textbf{k}_1,\,\textbf{k}_2,\,\textbf{k}_3}
\def\Bkkk{B(\kall)}
\def\Skkk{S(\kall)}

\def\Cl{C_\ell}
\def\alm{a_{\ell m}}
\def\almone{a_{\ell_1m_1}}
\def\almtwo{a_{\ell_2m_2}}
\def\almthree{a_{\ell_3m_3}}
\def\almfour{a_{\ell_4m_4}}
\def\almfive{a_{\ell_5m_5}}
\def\almsix{a_{\ell_6m_6}}
\def\Ylm{Y_{\ell m}}

\def\Vtetra{{{\cal V}_{\cal T}}}

\def\Q{\curl{Q}}
\def\Qn{\curl{Q}_n}
\def\Qm{\curl{Q}_m}
\def\Qp{\curl{Q}_p}
\def\Qnxyz{\curl{Q}_n(x,y,z)}

\def\R{\curl{R}}
\def\Rn{\curl{R}_n}
\def\Rm{\curl{R}_m}
\def\Rp{\curl{R}_p}
\def\Rnxyz{\curl{Q}_n(x,y,z)}

\def\barQ{\kern2pt\overline{\kern-2pt\curl{Q}}}
\def\barQn{\barQ_n}
\def\barQm{\barQ_m}
\def\barQp{\barQ_p}
\def\barQnxyz{\barQ_n(x,y,z)}

\def\bargamma{\kern2pt\overline{\kern-2pt\gamma}}
\def\barzeta{\kern2pt\overline{\kern-2pt\zeta}}

\def\barR{\kern2pt\overline{\kern-2pt\curl{R}}}
\def\barRn{\barR_n}
\def\barRm{\barR_m}
\def\barRp{\barR_p}
\def\barRnxyz{\barR_n(x,y,z)}

\def\nmax{n_\textrm{max}}

\def\aR{\alpha^{\scriptscriptstyle{\cal R}}}
\def\aRn{\aR_n}
\def\aRp{\aR_p}
\def\baR{\bar{\alpha}^{\scriptscriptstyle{\cal R}}}
\def\baRn{\baR_n}
\def\baRp{\baR_p}

\def\aQ{\alpha^{\scriptscriptstyle{\cal Q}}}
\def\aQn{\aQ_n}
\def\aQp{\aQ_p}
\def\baQ{\bar{\alpha}^{\scriptscriptstyle{\cal Q}}}
\def\baQn{\baQ_n}
\def\baQp{\baQ_p}

\def\bR{\beta^{\scriptscriptstyle{\cal R}}}
\def\bRn{\bR_n}
\def\bRp{\bR_p}
\def\bbR{\bar{\beta}^{\scriptscriptstyle{\cal R}}}
\def\bbRn{\bbR_n}
\def\bbRp{\bbR_p}

\def\bQ{\beta^{\scriptscriptstyle{\cal Q}}}
\def\bQn{\bQ_n}
\def\bQp{\bQ_p}
\def\bbQ{\bar{\beta}^{\scriptscriptstyle{\cal Q}}}
\def\bbQn{\bbQ_n}
\def\bbQp{\bbQ_p}

\def\Qndefn{q_{\{p}\,q_r\,q_{s\}}}
\def\bQndefn{\bar q_{\{p}\,\bar q_r\,\bar q_{s\}}}

%Map notations - equilateral and local models
\def\balpha{\mbox{\boldmath$\alpha$}_l}
\def\bbeta{\mbox{\boldmath$\beta$}_l}
\def\bgamma{\mbox{\boldmath$\gamma$}_l}
\def\bdelta{\mbox{\boldmath$\delta$}_l}
\def\Malpha{M_\alpha(x,\hat{\bf n})}
\def\Mbeta{M_\beta(x,\hat{\bf n})}
\def\Mgamma{M_\gamma(x,\hat{\bf n})}
\def\Mdelta{M_\delta(x,\hat{\bf n})}

\newcommand{\kv}{{\bf k}}
\def\alll{\ell_1 \ell_2 \ell_3}
\def\fnll{f_{\rm NL}^{\rm local}}

\def\threej#1#2#3#4#5#6{\left( \begin{array}{ccc} #1 & #2 & #3 \\ #4 & #5 & #6 \end{array} \right) }
\def\llist{\ell_1,\ell_2,\ell_3}
\def\klist{k_1,k_2,k_3}
\def\eqref#1{(\ref{#1})}

\def\leaderfi1{\leaders\hbox to 5pt{\hss.\hss}\hfil}

%% ANY LOCAL DEFINITIONS HERE 
%\def\initialauthors#1{\noindent {\it #1:}\\}


%FONT MODIFICATIONS
\def\setsize{\csname @setfontsize\endcsname \setsize}


==> CGM/results.tex <==
We use the estimator in \citet{DS2009} to reconstruct a fluctuating $\tau$ map, this map is then cross correlated with a given galaxy or cluster sample or with a Compton-$y$ map, which produces cross spectra ($C^{\tau g}_\ell$ and $C^{\tau y}_\ell$, respectively). A similar approach was proposed to measure the fluctuations in $\tau$ from reionzation by cross-correlating with measurements from 21cm experiments \citep{Meerburg2013}. The amplitude of cross spectra proposed here are directly proportional to the amplitude of the $\tau--y$ and $\tau--M$ relations. Even for measurements of $C^{\tau y}_\ell$, the measurements of $\langle y \rangle_\rmn{\Theta}$ will break degeneracies between $y$ and $\tau$. If we make a high significance measurement of these cross spectra then we can empirically calibrate the $\tau--y$ and $\tau--M$ relations and eliminate the systematic uncertainties from astrophysics.

We forecast the signal-to-noise ratio ($\rmn{S} / \rmn{N}$) of these cross spectra for future CMB experiments. The calculation of the noise power spectrum, $N_\ell^{\tau\tau}$, is describe in \citet{DS2009} and we only consider polarization estimator since the temperature estimator will be contaminated by kSZ signal. We use the simulations described in Section \ref{sec:sims} and analytic halo model calculations (See Appendix \ref{sec:halo}) to calculate the cross spectra $C^{\tau g}_\ell$ and $C^{\tau y}_\ell$. Here the field $g$ refer to a number-count map where a non-zero value is assigned at the location of each halo above a given minimum mass and $y$ is a Compton-$y$ map with the same mass threshold. We cross correlate the number-count and Compton-$y$ maps with the $\tau$ map at each simulation output for all the simulations. Then for each redshift we average over all simulations realizations and add these differential cross-spectra up to get the signal.

The total $\rmn{S} / \rmn{N}$ is calculated by summing the signal-to-noise per $\ell$ mode,

\be
\left(\rmn{S} / \rmn{N}\right)^2 = \sum_\ell{\left(\frac{C_\ell^{\tau i}}{\Delta C_\ell^{\tau i} }\right)^2},
\ee

\noindent where $\Delta C_\ell^{\tau i}$ is theoretical errors on $C_\ell^{\tau i}$ given a $N_\ell^{\tau\tau}$. The exact form of $\Delta C_\ell^{\tau i}$ we use is 

\be
\left (\Delta C_\ell^{\tau i} \right)^2 = \frac{1}{f_\rmn{sky}(2\ell + 1)} \left[N_\ell^{\tau\tau}\left(C_\ell^{ii} + N_\ell^{ii} \right)   \right],
\label{eq:delcl}
\ee

\noindent where $f_\rmn{sky}$ is the fraction of sky covered, $C_\ell^{ii}$ and $N_\ell^{ii}$ are the auto spectrum and shot noise term of a given tracer, respectively. Here we used that $N_\ell^{\tau\tau} >> C_\ell^{\tau\tau}$ to simple Equation \ref{eq:delcl}. We calculate $C_\ell^{ii}$ and $N_\ell^{ii}$ from the simulations and analytic halos models with the same parameters as $C^{\tau g}_\ell$ and $C^{\tau y}_\ell$.

%C_\ell^{ii} C_\ell^{\tau\tau} +  \left(C_\ell^{i,\tau}\right)^2   +

The amplitude and shape of $N_\ell^{\tau\tau}$ will depend on the experiment that we are forecasting for. We make forecasts for a CMB-S4 like survey that has a noise level of 1$\mu$K acrmin. The $\ell$ range we consider is from 100-5000 in polarization and we choose two full-width half max beam sizes of 1 and 3 arcmins. In Figure \ref{fig:SN} we the show the total $\rmn{S} / \rmn{N}$ as a function of $\ell$. For a halo mass threshold of $M_{500} > 3\times10^{13} M_\odot$ {\bf CHECK THIS} we find the total $\rmn{S} / \rmn{N} f_\rmn{sky}^{-1/2} = 18\sigma$ and $20\sigma$ for $C^{\tau g}_\ell$ and $C^{\tau y}_\ell$, respectively. Here the halo mass threshold is at lower limit on the simulations. Such a measurement would place 6-8\% percent calibration on $\tau--y$ and $\tau--M$ relations for a full sky CMB-S4 experiment. A more conservative forecast with $f_\rmn{sky} = 0.4$ will calibrate the $\tau--y$ and $\tau--M$ relations to better than 9-12\%.

With the analytic halo model we are not subject to such a mass threshold and push the calculation to lower halo masses. We gain {\bf (or loose)} $\rmn{S} / \rmn{N}$ here because of {\bf BLANK MORE}. 


.... 


==> results.tex <==
We use the estimator in \citet{DS2009} to reconstruct a fluctuating $\tau$ map, this map is then cross correlated with a given galaxy or cluster sample or with a Compton-$y$ map, which produces cross spectra ($C^{\tau g}_\ell$ and $C^{\tau y}_\ell$, respectively). A similar approach was proposed to measure the fluctuations in $\tau$ from reionzation by cross-correlating with measurements from 21cm experiments \citep{Meerburg2013}. The amplitude of cross spectra proposed here are directly proportional to the amplitude of the $\tau--y$ and $\tau--M$ relations. Even for measurements of $C^{\tau y}_\ell$, the measurements of $\langle y \rangle_\rmn{\Theta}$ will break degeneracies between $y$ and $\tau$. If we make a high significance measurement of these cross spectra then we can empirically calibrate the $\tau--y$ and $\tau--M$ relations and eliminate the systematic uncertainties from astrophysics.

We forecast the signal-to-noise ratio ($\rmn{S} / \rmn{N}$) of these cross spectra for future CMB experiments. The calculation of the noise power spectrum, $N_\ell^{\tau\tau}$, is describe in \citet{DS2009} and we only consider polarization estimator since the temperature estimator will be contaminated by kSZ signal. We use the simulations described in Section \ref{sec:sims} and analytic halo model calculations (See Appendix \ref{sec:halo}) to calculate the cross spectra $C^{\tau g}_\ell$ and $C^{\tau y}_\ell$. Here the field $g$ refer to a number-count map where a non-zero value is assigned at the location of each halo above a given minimum mass and $y$ is a Compton-$y$ map with the same mass threshold. We cross correlate the number-count and Compton-$y$ maps with the $\tau$ map at each simulation output for all the simulations. Then for each redshift we average over all simulations realizations and add these differential cross-spectra up to get the signal.

The total $\rmn{S} / \rmn{N}$ is calculated by summing the signal-to-noise per $\ell$ mode,

\be
\left(\rmn{S} / \rmn{N}\right)^2 = \sum_\ell{\left(\frac{C_\ell^{\tau i}}{\Delta C_\ell^{\tau i} }\right)^2},
\ee

\noindent where $\Delta C_\ell^{\tau i}$ is theoretical errors on $C_\ell^{\tau i}$ given a $N_\ell^{\tau\tau}$. The exact form of $\Delta C_\ell^{\tau i}$ we use is 

\be
\left (\Delta C_\ell^{\tau i} \right)^2 = \frac{1}{f_\rmn{sky}(2\ell + 1)} \left[N_\ell^{\tau\tau}\left(C_\ell^{ii} + N_\ell^{ii} \right)   \right],
\label{eq:delcl}
\ee

\noindent where $f_\rmn{sky}$ is the fraction of sky covered, $C_\ell^{ii}$ and $N_\ell^{ii}$ are the auto spectrum and shot noise term of a given tracer, respectively. Here we used that $N_\ell^{\tau\tau} >> C_\ell^{\tau\tau}$ to simple Equation \ref{eq:delcl}. We calculate $C_\ell^{ii}$ and $N_\ell^{ii}$ from the simulations and analytic halos models with the same parameters as $C^{\tau g}_\ell$ and $C^{\tau y}_\ell$.

%C_\ell^{ii} C_\ell^{\tau\tau} +  \left(C_\ell^{i,\tau}\right)^2   +

The amplitude and shape of $N_\ell^{\tau\tau}$ will depend on the experiment that we are forecasting for. We make forecasts for a CMB-S4 like survey that has a noise level of 1$\mu$K acrmin. The $\ell$ range we consider is from 100-5000 in polarization and we choose two full-width half max beam sizes of 1 and 3 arcmins. In Figure \ref{fig:SN} we the show the total $\rmn{S} / \rmn{N}$ as a function of $\ell$. For a halo mass threshold of $M_{500} > 3\times10^{13} M_\odot$ {\bf CHECK THIS} we find the total $\rmn{S} / \rmn{N} f_\rmn{sky}^{-1/2} = 18\sigma$ and $20\sigma$ for $C^{\tau g}_\ell$ and $C^{\tau y}_\ell$, respectively. Here the halo mass threshold is at lower limit on the simulations. Such a measurement would place 6-8\% percent calibration on $\tau--y$ and $\tau--M$ relations for a full sky CMB-S4 experiment. A more conservative forecast with $f_\rmn{sky} = 0.4$ will calibrate the $\tau--y$ and $\tau--M$ relations to better than 9-12\%.

With the analytic halo model we are not subject to such a mass threshold and push the calculation to lower halo masses. We gain {\bf (or loose)} $\rmn{S} / \rmn{N}$ here because of {\bf BLANK MORE}. 


.... 

